A Minimum Energy Filter for Localisation of an Unmanned Aerial Vehicle

Accurate localisation of unmanned aerial vehicles is vital for the next generation of automation tasks. This paper proposes a minimum energy filter for velocity-aided pose estimation on the extended special Euclidean group. The approach taken exploits the Lie-group symmetry of the problem to combine Inertial Measurement Unit (IMU) sensor output with landmark measurements into a robust and high performance state estimate. We propose an asynchronous discrete-time implementation to fuse high bandwidth IMU with low bandwidth discrete-time landmark measurements typical of real-world scenarios. The filter's performance is demonstrated by simulation.

==> filter_derivation/macros.tex <==

% Special Euclidean group
\newcommand{\SE}{\mathrm{SE}}
\newcommand{\se}{\mathfrak{se}}
\newcommand{\SO}{\mathrm{SO}}
\newcommand{\so}{\mathfrak{so}}
\newcommand\Tau{\mathrm{T}}
\newcommand{\inv}{^{\text{-}1}}

\newcommand*{\Real}[1]{\ensuremath{\mathbb{R}^{#1}}}

\newcommand\norm[1]{\ensuremath{\left\Vert #1 \right\Vert}}
\newcommand\proj[1]{\ensuremath{\mathbb{P}\left( #1 \right)}}
\newcommand\projsym[1]{\ensuremath{\mathbb{P}_s\left( #1 \right)}}
\newcommand\projasym[1]{\ensuremath{\mathbb{P}_a\left( #1 \right)}}


\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\blkdiag}{blkdiag}
\DeclareMathOperator{\eigvecs}{eigvecs}
\DeclareMathOperator{\eigvals}{eigvals}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\vex}{vex}
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator\Hess{Hess}
\bmdefine{\der}{\mathrm{d}}

\newcommand{\doubleplus}{\mathrel{+\!\!\!+}}


==> filter_derivation/main.tex <==
\include{preamble}
\include{macros}

\begin{document}
%\section{Global State Filter - Problem Formulation}
\subsection{Preliminaries}
\begin{align}
	\begin{bmatrix} \omega \\ a \\ v \end{bmatrix}^\wedge
    &= \begin{bmatrix}\omega_\times & a & v \\ 0 & 0 & 0 \\ 0 & 0 & 0 \end{bmatrix} \in\se_2(3), (\omega, a, v \in \Real{3})
	\\
	 \begin{bmatrix}\omega_\times & a & v \\ 0 & 0 & 0 \\ 0 & 0 & 0 \end{bmatrix}^\vee
    &= \begin{bmatrix}\omega \\ a \\ v \end{bmatrix}
    \\
    \bar{a} &= \begin{bmatrix}
        a \\ 0 \\ 1
    \end{bmatrix}
    , a \in \Real{3}
    \\
%    \bar{A} &= \begin{bmatrix}
%    A & 0 \\ 0 & 1
%    \end{bmatrix}
%    , A \in \Real{n \times n}
%    \\
%    \mathring{a} &= \begin{bmatrix}a \\ 0 \end{bmatrix}, a \in \Real{3}
%    \\
	F &: \Real{3} \rightarrow \mathcal{L}(\Real{9}, \Real{5})
	\\
	F(v) &:= \begin{bmatrix} -v_\times & 0 & I_3 \\ 0 & 0 & 0 \\ 0 & 0 & 0 \end{bmatrix}
	\\
	X \bar{v} &= F(v) X^\vee
	\\
    G &: \Real{3} \rightarrow \mathcal{L}(\Real{9}, \Real{5})
    \\
    G(v) &:= \begin{bmatrix} v_\times & 0 & 0 \\ 0 & v^\top & 0 \\ 0 & 0 & v^\top \end{bmatrix}
    \\
    X^\top \bar{v} &= G(v) X^\vee
\end{align}
%
%\subsection{Robot Kinematics}
%For each robot $i \in [1, \ldots, n]$ the pose kinematics of the vehicle is given by:
%\begin{align}
%	X_i &= \begin{bmatrix}R_i & p_i\\ 0 & 1\end{bmatrix} \in \SE(3)
%	\\
%	\dot{X}_i &= X_i \begin{bmatrix}\omega_i \\ v_i\end{bmatrix}^\wedge
%\end{align}
%We concatenate the poses of each robot to form the global state tuple, $Z$:
%\begin{align}
%	Z &= \left( X_1, X_2, \ldots, X_n \right)
%	\\
%	\dot{Z}
%    &= Z  \odot \left(\begin{bmatrix}\omega_1\\v_1\end{bmatrix}, \begin{bmatrix}\omega_2\\v_2\end{bmatrix}, \ldots, \begin{bmatrix}\omega_n\\v_n\end{bmatrix} \right)^\wedge
%\end{align}
%where $\odot$ is element-wise matrix multiplication and $(\cdot)^\wedge$ is applied element-wise.
%
%\subsection{Interoceptive Measurements}
%Each robot is capable of measuring its own angular and linear velocities.
%\begin{align}
%u_i &= \begin{bmatrix}
%\omega_i \\
%v_i
%\end{bmatrix} + B_i\epsilon_i
%\end{align}
%where $\epsilon_i \in \Real{6}$ is the measurement error, characterised by $ B_i \in \Real{6 \times 6}$. Thus, we can construct a global measurement vector:
%\begin{align}
%u &= \left(u_1, u_2, \ldots, u_n\right)
%\end{align}
%
%\subsection{Communications Network}
%Robots are able to communicate to each other over a network. The communication links between the $n$ robots in the system can be represented as a directed graph, $G(t) = (V, E(t))$. $V = \{1, \ldots, n\}, E \subseteq \left(V \times V\right)$.  If $(i, j) \in E(t)$ then $i$ can recieve message from $j$ at time $t$.
%
%$\Tau_i = \{\tau_{i1}, \ldots, \tau_{ik_t} \}  \subset (0,t), k_t \in \mathbb{N}$ is the finite set of times where vehicle $i$ receives a message.
%
%Robot $j$ sends a message to robot $i$ about the estimated position of a point fixed to $j$. The message received,  $s_{ij}$, by robot $i$ from robot $j$ is defined as:
%\begin{align}
%    \bar{s}_{ij} &= \hat{X}_j\bar{l}_{j} + X_i \bar{G}_{ij} \bar{\eta}_{ij}
%\end{align}
%where $l_{j} \in \Real{3}$ is a known fixed point on the robot $j$, $\eta \in \Real{3}$ is the noise introduced by the communication process, characterised by $G_{ij} \in \Real{3\times3}$
%
%In the recieved message, $i$ receives information about robot $j$'s own estimate of their pose, $\hat{X}_j$. However, there is also an error between this estimate and the true state:
%\begin{align}
%\hat{X}_j \bar{l}_j &= X_j \bar{l_j} + X_i \bar{Q}_{ij} \bar{\xi}_{ij}
%\end{align}
%
%where $\xi_{ij} \in \Real{3}$, characterised by $Q_{ij} \in \Real{3 \times 3}$.
%
%In the global estimation problem, communication between robots is not required as all robot pose estimates are known. However, $\Tau_i$ also represents the times at which exteroceptive measurements are acquired.
%
%\subsection{Exteroceptive Measurements}
%A robot is capable of taking a vector measurement to a known point, $l$, fixed to the robot. $y_{ij}$ is a measurement taken by $i$ to a point $l_j$ on robot $j$.
%\begin{align}
%y_{ij} &= X_i^{-1} X_j \bar{l}_j + \bar{D}_{ij} \bar{\delta}_{ij}
%\end{align}
%where $\delta_{ij} \in \Real{3}$ is the measurement noise, characterised by $D \in \Real{3 \times 3}$.
%
%%
%%$x_i |_{(0,t)} \in \SE(3)$ is the trajectory of vehicle $i$.
%%
%%$u_i |_{(0,t)} = [\Omega, V]^\top + \omega \in \se(3)$ is the velocity measurements of vehicle $i$.
%%
%%$\hat{x}_i(t) \in \SE(3)$ is the estimate of the state $x_i(t)$.
%%
%%$y_{ij} := x_i^{-1} x_j P_j + \delta_{ij}$ is the measurement vehicle $i$ makes of the point, $P_j$, which is in the BFF of vehicle $j$.
%
%
%
%\subsection{Global State Estimate Problem}
%
%Determine $\hat{Z}(t), H(t)$ that minimises the cost functional:
%
%\begin{gather}
%J = \norm{Z(0) - \hat{Z}(0)}^2_{H^{-1}(0)} + \frac{1}{2} \int_{0}^{t} \sum_{i=1}^{n} \norm{\epsilon_i(\tau)}^2 d\tau\\
%J^+ = J + \frac{1}{2} \norm{\bar{\delta}_{ij}(\tau_{ik})}^2
%\end{gather}
%
%given $u|_{(0,t)}$ and $\{y_{ij}( \tau_{ik}) | (i,j) \in E(t), \tau_{ik} \in T_i \}$
%
%\subsection{Decentralised State Estimate Problem}
%
%For each robot, determine $\hat{X}_i(t), \Sigma_i(t)$ that minimises the cost functional:
%\begin{align}
%J_i &= \norm{X_i(0) - \hat{X}_i(0)}^2_{\Sigma_i^{-1}(0)} + \frac{1}{2}\int_0^t \norm{\epsilon_i(\tau)}^2 d\tau\\
%J^+ &= J + \frac{1}{2}\left( \norm{\delta_{ij}(\tau_{ik})}^2 + \norm{\eta_{ij}(\tau_{ik})}^2 + \norm{\xi_{ij}(\tau_{ik})}^2 \right)
%\end{align}
%
%given  $u_i|_{(0,t)}$ and $\{\left( y_{ij}( \tau_{ik}), m_{ij}( \tau_{ik}) \right)  | (i,j) \in E(t), \tau_{ik} \in T_i \}$
%
%\subsection{Research Problem}
%Given that the decentralised filter does not account for the entire covariance matrix, an estimation of the cross correlation terms must be made. The aim is to characterise the performance of both the centralised and decentralised filters and examine how the loss of information about the cross correlations affects the decentralised filter. Long term, this should allow us to make an informed decision about the best way to estimate the missing terms and what information needs to be communicated between robots.
%
%
%\newpage

\section{GAME Filter for SE(3) with velocity}

\subsection{Vehicle Kinematics}

Consider a rigid-body vehicle in free space. The position, $x \in \Real{3}$, orientation, $R \in \SO(3)$, and linear velocity, $v \in \Real{3}$ of the body-fixed frame with respect to the inertial frame are all expressed in the coordinates of the inertial frame.

The kinematics of the vehicle is given by
\begin{align}
\dot{R} &= R \omega_\times
\\
\dot{v} &= R a
\\
\dot{x} &= v
\end{align}
where $\omega \in \Real{3}$ is the angular velocity, and $a \in \Real{3}$ is the linear acceleration of the body-fixed frame with respect to the inertial frame, expressed in the body-fixed frame.

The vehicle state, $g$, can be expressed as a matrix group, often referred to as $\SE_2(3) \subset \Real{5\times5}$
\begin{align}
g &= \begin{bmatrix}
R & v & x \\ 0 & 1 & 0 \\ 0 & 0 & 1
\end{bmatrix}
\intertext{which yields the following matrix-group kinematics}
\dot{g} &= g \begin{bmatrix}\omega_\times & a & R^\top v \\ 0&0&0 \\ 0&0&0 \end{bmatrix}, \quad g(t_0) = g_0
\end{align}


The vehicle is equipped with an IMU, which measures linear acceleration $u_a$ and angular velocity, $u_\omega$, in the body-fixed frame. The measurements are modelled by
\begin{align}
u_\omega &= \omega + B_\omega \delta_\omega
\\
u_a &= a + B_a \delta_a
\end{align}
where $\delta_\omega \in \Real{3}, \delta_a \in \Real{3}$ are unknown error signals assumed to be zero mean and square integrable.

Substituting the measurement model into the kinematics gives
\begin{align}
\dot{g} &= g \left( \begin{bmatrix}(u_{\omega})_\times & u_a & R^\top v \\ 0 & 0 & 0 \\ 0 & 0 & 0 \end{bmatrix} + \begin{bmatrix} (-B_\omega \delta_\omega)_\times & -B_a \delta_a & 0 \\ 0 & 0 & 0 \\ 0 & 0 & 0 \end{bmatrix} \right)
\\
&= g \left( \lambda_t(g, u) + B(\delta_t )\right)
\\
&= g \left( \begin{bmatrix}u_\omega \\ u_a \\ R^\top v \end{bmatrix} + \begin{bmatrix} -B_\omega & 0 \\ 0 & - B_a \\ 0 & 0 \end{bmatrix} \begin{bmatrix}
\delta_\omega \\ \delta_a
\end{bmatrix} \right) ^\wedge
\end{align}

\subsection{Landmark Measurements}
The vehicle is equipped with a sensor that measures relative translations to a fixed landmark, $l \in \Real{3}$ in the environment. The measurement model is given by
\begin{align}
y(t) &= R^\top(l - x) + D \epsilon_t
\\
&= h_t(g) + D \epsilon_t
\end{align}
where $\epsilon \in \Real{3}$ is the unknown measurement error. 

\subsection{Minimisation Problem}
Consider the following cost function on the system
\begin{align}
J_t &= % d_{P_0}(X_0, \hat{X}(0)) + \norm{v_0 - \hat{v}(0)}^2 + \norm{b_{\omega} (0) - \hat{b}_{\omega} (0)}^2 
\frac{1}{2} m_0(g_0) + \frac{1}{2} \int_{t_0}^t \norm{\delta_\tau}^2 + \norm{\epsilon_\tau}^2 d\tau 
\end{align}
We define the minimising trajectory $g^*_{[t_0, t]}$ as the trajectory which is compatible with the system kinematics and measurement model and that minimises $J_t$.

The filter estimate, $\hat{g}$, is defined as the terminal point of the minimising trajectory over the time period $[t_0, t]$ i.e. $\hat{g}(t) = g^*_{[t_0, t]}(t)$.

\subsection{Filter Derivation}
From Saccon et al., the second-order optimal filter for the system described is given by
\begin{align}
\dot{\hat{g}} &= \hat{g} \left( \lambda_t(\hat{g}, u) + K(t) r_t(\hat{g}) \right), \quad \hat{g}(t_0) = \hat{g}_0
\\
\intertext{with the following definitions}
\hat{g}_0 &= \argmin_g m_0(g)
\\
r_t(\hat{g}) &= T_eL^*_{\hat{g}} \circ \left[ \left( P_y \circ (y - \hat{y}) \right) \circ \der h_t(\hat{g}) \right]
\\
P_y &=  (D\inv)^* \circ D\inv, \quad \hat{y} = h_t(\hat{g})
\\
\dot{K} &= A \circ K + K \circ A^* - K \circ E \circ K + B \circ  B^* - \omega_{Kr} \circ K - K \circ \omega^*_{Kr}
\\
K(t_0) &= X_0\inv
\\
X_0 &= T_eL^*_{\hat{g}_0} \circ \Hess m_0(\hat{g}_0) \circ T_eL_{\hat{g}}
\\
A(t) &=\der_1 \lambda_t(\hat{g}, u) \circ T_eL_{\hat{g}} - \ad_{\lambda_t(\hat{g}, u)} - T_{\lambda_t(\hat{g}, u)}
\\
E(t) &= - T_eL^*_{\hat{g}} \circ \left[ \left( P_y \circ (y - \hat{y}) \right) ^ {T_{\hat{g}}G} \circ \Hess h_t(\hat{g}) - (\der h_t(\hat{g}))^* \circ P_y  \circ \der h_t(\hat{g}) \right] \circ T_eL_{\hat{g}}
\end{align}


\subsection{Adjoint Representation}
The adjoint representation of the lie algebra is equal to the lie bracket operator. For $X, Y \in \se_2(3)$
\begin{align}
\ad_X Y &= [X, Y]
\\
&= XY - YX 
\\
&= \begin{bmatrix}
X_{\omega\times} Y_{\omega\times}  - Y_{\omega\times} X_{\omega\times} &
X_{\omega\times} Y_a - Y_{\omega\times}X_a  & 
X_{\omega\times} Y_v - Y_{\omega\times} X_v \\
0 & 0 & 0\\
0 & 0 & 0 
\end{bmatrix}
\\
&= \begin{bmatrix}
(X_{\omega\times} Y_{\omega})_\times&
X_{\omega\times} Y_a + X_{a\times} Y_{\omega}  & 
X_{\omega\times} Y_v + X_{v\times} Y_{\omega} \\
0 & 0 & 0\\
0 & 0 & 0 
\end{bmatrix}
\intertext{The matrix representation is then}
\ad_X &= \begin{bmatrix}
X_{\omega\times} & 0 & 0 \\
X_{a\times} & X_{\omega\times} & 0 \\
X_{v\times} & 0 & X_{\omega\times}
\end{bmatrix}
\end{align}

\subsection{Connection Function}
We use the Cartan (0)-Connection, which, for $X, Y \in \se_2(3)$, is defined as
\begin{align}
\omega_X(Y) &:= \frac{1}{2} [X, Y]
\\
\omega_X &= \frac{1}{2}\ad_X
\\
\intertext{For the chosen connection, the torsion tensor is zero}
T_X = 0
\end{align}

\subsection{Derivative of measurement function}
\begin{align}
h_t(g) &= R^\top (l - x)
\\
\bar{h}_t(g) &= g\inv \bar{l}
\\
\der \bar{h}_t(g) \circ g X &= - g\inv g X g\inv \bar{l}
\\
&= - X \bar{h}_t(g)
\\
&= - F(\hat{y}) X^\vee
\\
\der h_t(g) \circ g X &= \begin{bmatrix}\hat{y}_\times & 0 & -I_3 \end{bmatrix} X^\vee
\end{align}

\begin{align}
\Hess h_t(g) (gX) (gY) &= \der (\der h_t(g) \circ gY) \circ gX - \der h_t(g) \circ g \omega_X(Y)
\\
&= - \der Y g\inv \bar{l} \circ gX + \frac{1}{2} [X,Y] \bar{h}_t(g)
\\
&= YX h_t(g) + \frac{1}{2} XY h_t(g) - \frac{1}{2} YX h_t(g)
\\
&= \frac{1}{2} \left(XY h_t(g) + YX h_t(g)\right) 
\end{align}


\subsection{Residual}
\begin{align}
r_t(\hat{g}) &= T_eL^*_{\hat{g}} \circ \left[ \left( P_y \circ (y - \hat{y}) \right) \circ \bm{d}h_t(\hat{g}) \right]
\\
r_t(\hat{g}) \circ X &= \left( P_y \circ (y - \hat{y}) \right) \circ \bm{d}h_t(\hat{g}) \circ gX
\\
&=\left( P_y \circ (y - \hat{y}) \right) \circ  \begin{bmatrix}\hat{y}_\times & 0 & -I_3 \end{bmatrix} X^\vee
\\
r_t(\hat{g}) &= \left( P_y \circ (y - \hat{y}) \right)^\top  \begin{bmatrix}\hat{y}_\times & 0 & -I_3 \end{bmatrix}
\end{align}

\subsection{A(t)}
\begin{align}
\der_1 \lambda_t(\hat{g}, u) \circ gX &= \der_1  \begin{bmatrix}(u_{\omega})_\times & u_a & R^\top v \\ 0 & 0 & 0 \\ 0 & 0 & 0 \end{bmatrix} \circ gX
\\
&= \begin{bmatrix}
0 & 0 & R^\top R X_a + (R X_{\omega\times})^\top v \\ 0 & 0 & 0 \\ 0 & 0 & 0
\end{bmatrix}
\\
&=  \begin{bmatrix}
0 \\ 0 \\ X_a - X_{\omega\times} R^\top v
\end{bmatrix}^\wedge
\\
&=\left(\begin{bmatrix}
0 & 0 & 0 \\ 0 & 0 & 0 \\ (R^\top v)_\times & I & 0
\end{bmatrix}
X^\vee \right)^\wedge
\\
 \der_1 \lambda_t(\hat{g}, u) \circ T_eL_{\hat{g}} &= \begin{bmatrix}
 0 & 0 & 0 \\ 0 & 0 & 0 \\ (R^\top v)_\times & I & 0
 \end{bmatrix}
 \\
 \ad_{\lambda_t(\hat{g}, u)} &= \begin{bmatrix}
 u_{\omega\times} & 0 & 0\\
 u_{a\times} &  u_{\omega\times} & 0 \\
 (R^\top v)_\times & 0 &  u_{\omega\times}
 \end{bmatrix}
 \\
 A(t) &= \der_1 \lambda_t(\hat{g}, u) \circ T_eL_{\hat{g}} - \ad_{\lambda_t(\hat{g}, u)} - T_{\lambda_t(\hat{g}, u)}
 \\
 &= \der_1 \lambda_t(\hat{g}, u) \circ T_eL_{\hat{g}} - \ad_{\lambda_t(\hat{g}, u)}
 \\
 &= \begin{bmatrix}
 -u_{\omega\times} & 0 & 0\\
 -u_{a\times} &  -u_{\omega\times} & 0 \\
 0 & I &  -u_{\omega\times}
 \end{bmatrix}
\end{align}

\subsection{E(t)}
\begin{align}
E(t) &= - T_eL^*_{\hat{g}} \circ \left[ \left( P_y \circ (y - \hat{y}) \right) ^ {T_{\hat{g}}G} \circ \Hess h_t(\hat{g}) - (\der h_t(\hat{g}))^* \circ P_y  \circ \der h_t(\hat{g}) \right] \circ T_eL_{\hat{g}}
\\
[E(t)\circ X]\circ Y &= - \left[ \left[ \left( P_y \circ (y - \hat{y}) \right) ^ {T_{\hat{g}}G} \circ \Hess h_t(\hat{g}) - (\der h_t(\hat{g}))^* \circ P_y  \circ \der h_t(\hat{g}) \right] \circ \hat{g} X \right] \circ \hat{g}Y
\\
&= - \left[ \left[ \left( P_y \circ (y - \hat{y}) \right) ^ {T_{\hat{g}}G} \circ \Hess h_t(\hat{g}) \right] \circ \hat{g} X \right] \circ \hat{g} Y \\
& \quad + \left[ \left[ (\der h_t(\hat{g}))^* \circ P_y  \circ \der h_t(\hat{g}) \right] \circ \hat{g} X \right] \circ \hat{g} Y
\\
&= -  \left( P_y \circ (y - \hat{y}) \right) \circ \left[\Hess h_t(\hat{g}) \circ \hat{g} X \right] \circ \hat{g} Y \\
&\quad + \left[P_y \circ \der h_t(\hat{g}) \circ \hat{g} X \right] \circ \left[ \der h_t(\hat{g}) \circ \hat{g} Y \right]
\\
&= -  \left( P_y \circ (y - \hat{y}) \right) \circ \frac{1}{2} \left(XY h_t(\hat{g}) + YX h_t(\hat{g})\right)  + \left[P_y \circ X \bar{h}_t(\hat{g}) \right] \circ  Y \bar{h}_t(\hat{g})
\\
&= - \frac{1}{2} X^* \left( P_y \circ (y - \hat{y}) \right) \circ  F(\hat{y}) Y^\vee    - \frac{1}{2} Y^* \left( P_y \circ (y - \hat{y}) \right) \circ  F(\hat{y}) X^\vee \\
&\quad + \left[P_y \circ F(\hat{y}) X^\vee \right] \circ F(\hat{y}) Y^\vee
\\
F(\hat{y}) &= \begin{bmatrix}-\hat{y}_\times & 0 & I_3 \end{bmatrix}
\\
&= - \left(\frac{1}{2} F(\hat{y})^* \circ G\left( P_y \circ (y - \hat{y}) \right) \circ X^\vee \right) \circ   Y^\vee   \\
& \quad - Y^\vee \circ \left(\frac{1}{2} G\left( P_y \circ (y - \hat{y}) \right)^* \circ F(\hat{y}) X^\vee \right) \\
&\quad + \left(F(\hat{y})^*\circ P_y \circ F(\hat{y}) \circ X^\vee \right) \circ  Y^\vee
\\
E(t) &= - \projsym{F(\hat{y})^* \circ G\left( P_y \circ (y - \hat{y}) \right)} + F(\hat{y})^*\circ P_y \circ F(\hat{y}) 
\end{align}

\end{document}
